Geometric Rates of Convergence for Kernel-based Sampling Algorithms

The rate of convergence of weighted kernel herding (WKH) and sequential Bayesian quadrature (SBQ), two kernel-based sampling algorithms for estimating integrals with respect to some target probability measure, is investigated. Under verifiable conditions on the chosen kernel and target measure, we establish a near-geometric rate of convergence for target measures that are nearly atomic. Furthermore, we show these algorithms perform comparably to the theoretical best possible sampling algorithm under the maximum mean discrepancy. An analysis is also conducted in a distributed setting. Our theoretical developments are supported by empirical observations on simulated data as well as a real world application.

==> Distributed.tex <==
\section{Distributed Kernel Herding}
\label{sec:Distributed}
In many cases, the search over the domain $\cX$ can be a bottleneck causing the herding algorithm to be too slow to be useful in practice. In this section, we develop a new herding algorithm that can be distributed over multiple machines and run in a streaming map-reduce fashion. We also provide convergence analysis for the same, using techniques developed in Section~\ref{sec:theory}.

The algorithm proceeds as follows. The domain $\cX$ is split onto $s$ machines uniformly at random. Each of the $s$ machines has access to only $\cX_i \subset \cX$, such that $\cup_i \cX_i = \cX$ and $\cX_i \cap \cX_j = \emptyset $ for $i \neq j$. Each machine runs its own herding algorithm (Algorithm~\ref{algo:wkh}) independently, by specializing~\eqref{eq:LMO} to do a restricted search over $\cX_i$, instead of $\cX$. Finally, the iterates being generated by each machine are sent to a central server machine which \emph{collates} the samples from different machines by running another copy of the same algorithm, with $\cX$ replaced by the discrete set of samples sent to the central server by the other machines. Finally, the best solution out of all the $s+1$ solutions is returned. The pseudo-code is illustrated in Algorithm~\ref{algo:distributed}.We now provide the convergence guarantees for this algorithm.

\begin{wrapfigure}{r}{0.5\textwidth}\vspace{-8mm}
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
	\caption{Distributed Kernel Herding: Dist($\cX$, $k$)}
	\label{algo:distributed}
	\centering
	\begin{algorithmic}[1]
		\STATE  \textbf{INPUT:}kernel function $k(\cdot,\cdot)$, number of iterations $k$
		\STATE Partition $\cX \supset \cX_i, i \in [s]$ uniformly at random and transmit $\cX_i$ to machine $i$
		\STATE //Receive solution sets
		\STATE $\sfG_i, \bw_i$ $\leftarrow$ WKH($\cX_i$, $k$)  // run in parallel $\forall i \in [s]$
		\STATE $\cY = \cup_i \sfG_i$
		\STATE $\sfG_{s+1}, \bw_{s+1} \leftarrow$ WKH($\cY$, $k$)
		\STATE $i^\star \leftarrow \argmin_{i \in [s+1]} g(\sfG_i,\bw_i)$
		\STATE return $\sfG_{i^\star}$, $\bw_{i^\star}$ 
		\end{algorithmic}
	\vspace{-0.1cm}
\end{algorithm}
\end{minipage}
\end{wrapfigure}

\begin{theorem}
	\label{thm:Distributed}  Under Assumption 1, with $r=1$, and Assumptions 2 and 3, if $\sfS_i$ is the sequence of iterates produced by Algorithm~\ref{algo:distributed}, the function $g(\cdot)$ converges as $\bbE \min_\bw g(\sfS_i ,\bw) \leq \exp(- \frac{i m_\omega}{r M_\Omega}) g(\emptyset, 0)$.  
\end{theorem}

\noindent
\emph{Proof Idea:} Note that the final set of filtered iterates outputted are the \emph{best} out of $(s+1)$ possible sequences.  The proof tracks the possibilities for $\sfS_1^\star$ when $\cX$ is split. The goal is to then show that under all possible scenarios, at least one of the sequences converges linearly. The convergence of individual sequences is based on the proof techniques used in proof of Theorem~\ref{thm:WKHLinear}. 

%\noindent
%\emph{Remark.} 
We remark that, for the more general case of $r>1$, our proof technique does not give a valuable convergence rate. 
I%n particular, our analysis yields $g(\sfS \cup \{\bx\}) \leq (1-C) g(\sfS) + \left( 1- \nicefrac{m_\omega}{2 M_\Omega} \right)$, which is not very meaningful. 
This could be an artifact of our proof technique, and improving it is an interesting open question for future research.
Also, while we presented the analysis for Distributed $\wkh$, by Corollary~\ref{cor:convergenceSBQ}, the same rate also holds for Distributed SBQ. %Furthermore, Theorem~\ref{thm:Distributed} says linear convergence holds in expectation, provided that $\cX$ is split uniformly at random. An interesting open question here is convergence under arbitrary splits, or smarter splits (possibly to tackle the case $r>1$).



==> Experiments.tex <==
\section{Experiments}\label{sec:Experiments}
\begin{wrapfigure}{r}{0.5\textwidth}\vspace{-6mm}
\begin{minipage}{0.5\textwidth}
	\centering
	\includegraphics[scale=0.5]{simulated}
	\caption{Simulated data results for distributed SBQ/WKH. Herding is WKH with uniform weights. SBQ/WKH are single machine algorithms, while SBQ-5/WKH-5 are their respective distributed versions.}
	\label{fig:simulated}
\end{minipage}\vspace{-10mm}
\end{wrapfigure}

We refer the readers to earlier works for empirical evidence of the relative performance of the Herding and SBQ algorithms~\cite{Bach2012Herding,Chen2010SuperSamples,Welling2010,Welling2009a,Welling2009b,Huszar2012OptimallyWeightedHI,Ghahramani2002BayesianMC}.
In this section, we focus on studying the distributed versions of these algorithms to illustrate the speedup vs the accuracy tradeoff.% We perform a simulated study as well as a real world application of data summarization using coresets on three different datasets of varying sizes.

\subsection{Matching a Distribution}
In this study, our goal is to show the tradeoff between performance vs scalability when WKH/SBQ are distributed over multiple machines. Towards this end, we extend an experiment considered by~\cite{Chen2010SuperSamples,Huszar2012OptimallyWeightedHI}. In this experiment, the target density is a mixture of $20$ two dimensional Gaussian distributions. Samples are chosen by the contending algorithms, and the MMD distance of the sample distribution to the target distribution is reported for different number of samples. %It has been observed that SBQ performs better than WKH, which in turns performs better than uniformly weighted Herding. This is in line with theory.

The sampling subroutine (step 4 in Algorithm~\ref{algo:wkh}), requires solving an optimization problem over a continuous domain. To make the problem easier,~\cite{Chen2010SuperSamples,Huszar2012OptimallyWeightedHI} first select 10000 points uniformly at random as the set of potential candidates. They note that this does not affect the performance of chosen samples by much. We also adopt the same methodology with the additional step of arbitrarily partitioning these 10000 points over $m$ machines for $m=1,5$ to run Algorithm~\ref{algo:distributed} with the goal of studying the degradation of performance due to the partitioning. 

The results are reported in Figure~\ref{fig:simulated}. SBQ-5 and WKH-5 are distributed versions of SBQ and WKH respectively run over $5$ machines. The labels SBQ and WKH are for their respective single machine versions. Since the search space is split and the search step is parallelized, we get about 5X speedup in the algorithms, with a graceful degradation in the reported MMD. We noticed a similar pattern of degradation for larger number of machines but is omitted from the graph to avoid overcrowding.

\subsection{Data Summarization}
\vspace{-2mm}
In this section, we apply Algorithm~\ref{algo:distributed} to the task of data summarization under logistic regression, as considered by~\cite{HugginsCB16}. The task of data summarization is as follows. The goal is to select a few data samples that represent the data distribution \emph{sufficiently} well, so that a model built on the selected subsample of the training data does not degrade too much in performance on unseen test data. More specifically, we are interested in approximating the test distribution (i.e., discrete $p$) using a few samples from the training set. Hence, algorithms such as SBQ and WKH are applicable, provided we have a reasonable kernel function. Recently,~\cite{Khanna2019} used SBQ with Fisher Kernels~\cite{Jaakkola1999} for this task. By using the distributed SBQ/WKH over $m$ machines,  we obtain ${\sim}m$ times speedup on the run time with minimal loss in the log-likelihood of the selected sample when compared to the results of~\cite{Khanna2019} for this task across three different datasets namely \texttt{ChemReact}, \texttt{CovType} and \texttt{WebSpam}. %We use Fisher kernels~\cite{Jaakkola1999}, since they were recently used to show strong performance for this task~\cite{Khanna2019}. For completeness, we provide a brief overview of the Fisher kernel in the appendix.


The results are presented in Figure~\ref{fig:coresets}. The algorithms we run are WKH, SBQ, $m$-SBQ and $m$-WKH, where $m$ represents the number of machines used to select $k$ samples for different values of $k$. The m-WKH-1 experiment is obtained by using only the output of a single split out of $m$ of the dataset run on only one of the machines (as was done by~\cite{Khanna2019} to scale up since they do not have the distributed algorithm to work with). For completeness, we also include ``Random'' which selects the data points uniformly at random, and ``Coreset'' which was proposed by~\cite{HugginsCB16}. Additional details of the experimental setup are in Section~\ref{sec:ExperimentsAppendix} in the supplement.

%
%An interesting practical consideration between SBQ and WKH is that the inner subproblem~\eqref{eq:LMO_SBQ} is harder than~\eqref{eq:LMO}, not just in time complexity but also in its memory requirement. 
%This is because solving ~\eqref{eq:LMO_SBQ} will make repeated calls to calculate dot products across iterations, and this can rack up the run time quickly if the kernel matrix is pre-computed and stored in memory. 
%On the other hand,~\eqref{eq:LMO} does not have this shortcoming, and the kernel dot product can be calculated as required without significantly impacting the runtimes. 
%\section{Conclusion}\label{sec:Conclusion}

%mention that the linear convergence chapter is closed. 
%
\vspace{-1mm}
\paragraph{Conclusion:} 

We have presented novel analysis for two commonly used algorithms as well as for a new distributed algorithm for estimating means. 
Our results bridge the gap between theory and empirical evidence by presenting the fastest known convergence rates for these algorithms. 
Our realizability assumption is the key insight that allows us to improve upon previous results and also provide the new distributed algorithm. %, and at the same time we provide sufficient conditions for convergence in the pathological infinite dimensional case. 
There are quite a few interesting future research directions. 
An important one is studying convergence for the distributed algorithm for the case with realizability $r>1$. 
Can the realizability help in proposing other faster variants? 
Alternatively, what are the \emph{best} possible rates for these problems? 
.% in these and other related directions. 



\begin{figure}[H]
	\begin{subfigure}[b]{0.45\textwidth}
		%\centering
		\includegraphics[width=7cm, height=4.5cm]{chemreact}
		\caption{\texttt{ChemReact}}
	\end{subfigure}\hspace{10mm}
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=7cm, height=4.5cm]{covtype}
		\caption{\texttt{CovType}}
	\end{subfigure}	
	\newline
	\vspace{2mm}
	\begin{subfigure}[b]{\textwidth}
		\centering
		\includegraphics[width=7cm, height=4.5cm]{webspam}
		\caption{\texttt{WebSpam}}
	\end{subfigure}
	
	\caption{Performance for logistic regression over three datasets for variants of sampling methods. `Full' reports the numbers for training with the entire training set. The distributed versions of SBQ/WKH show minimal loss in accuracy while achieving almost linear speedup.}
	\label{fig:coresets}
\end{figure}
%
%\newpage
%\section{Broader Impact}
%The primary nature of this work is theoretical. It provides a novel way to prove convergence rates, that has not been used before (and could be of independent interest), and explains the strong empirical performance of already known algorithms. This work also provides a new parallel algorithm that scales to much bigger datasets and thus, enhances the scope of herding algorithms. We hope that this motivates further research into scaling up sampling algorithms. This opens the door for possible future works into federated learning or serverless settings. We are not aware of any negative impacts of this work. 


==> Introduction.tex <==
\section{Introduction} \label{sec:intro}

Estimating expectations of functions is a common problem that is fundamental to many applications in machine learning, e.g., computation of marginals, prediction after marginalization of latent variables, calculating the risk, bounding the generalization error, estimating sufficient statistics, etc. 
In all these cases, the goal is to approximate tractably the~integral 
\begin{equation}
\bbE_p[f(\bx)] = \int_\cX f(\bx)p(\bx)d\bx ,
\label{eq:expectation}
\end{equation}
for a given function $f(\cdot)$, with value oracle access, and density $p$, with sampling oracle access. 
In most cases of interest, the integral is not computable in closed form. 
A common solution is to sample from the domain of $f(\cdot)$, and then to approximate the full integration using the samples. 
The simplest version of this is to use vanilla Monte Carlo (MC) Integration---sample uniformly at random from the domain of $f(\cdot)$, and then output the empirical average as the estimate of the integral. 
This simple algorithm converges at a prohibitively slow rate of $O(1/T)$ for squared distance of from the true mean.
More generally, one can apply Markov Chain Monte Carlo (MCMC) algorithms for~\eqref{eq:expectation}, and these algorithms come with many benefits, but they also converge quite slowly.

To alleviate the slower convergence of MC-based Integration, non-uniformly at random sampling algorithms such has Kernel Herding (KH) have been proposed. 
The herding algorithm~\cite{Welling2009a,Welling2009b,Welling2010} was proposed to learn Markov Random Fields (MRFs), and it was applicable to discrete finite-dimensional spaces. 
This was extended to continuous spaces and infinite dimensions using the kernel trick by~\cite{Chen2010SuperSamples}, who also provided a convergence rate of $O(1/T)$, which is theoretically the same as convergence rate of MC Integration in general. However, in practice, it has been observed that herding is faster. 
The speed up can be attributed to a smarter selection of sampling points (rather than uniformly at random) that ensures that the selected samples are somewhat negatively correlated.
In addition, \cite{Chen2010SuperSamples} also provided a \emph{moment matching} interpretation of the algorithm. 
Essentially, solving~\eqref{eq:expectation} using the weighted average of a few samples ($\bx_i$) can be interpreted as minimizing a discrepancy in an Reproducing Kernel Hilbert Space (RKHS). 
The discrepancy is also widely known to be the Maximum Mean Discrepancy (MMD) metric~\cite{Chen2010SuperSamples,Huszar2012OptimallyWeightedHI}.

In an alternative Bayesian approach,~\cite{Ohagan1991,Ghahramani2002BayesianMC} assume a Gaussian Process prior on $f(\cdot)$ and use a herding algorithm to sample so as to minimize the corresponding moment matching discrepancy arising out of the posterior of $f(\cdot)$, after observing the points already sampled. 
This perspective was shown to be equivalent to minimizing the herding discrepancy, but with an additional step of also minimizing the weights attached to the sampled points, instead of using uniform weights of $\nicefrac{1}{n}$~\cite{Huszar2012OptimallyWeightedHI}. 
Empirically, it was observed that this new algorithm---called Sequential Bayesian Quadrature (SBQ)---converges faster than naive herding because of the additional weight optimization step. 
To the best of our knowledge, the analysis of faster convergence for SBQ was still largely an open problem before our present~work.

A partial explanation for faster convergence in Weighted Kernel Herding (WKH) was provided by~\cite{Bach2012Herding}. While SBQ chooses the next sample point and the weights to minimize the said discrepancy, the herding algorithm only solves a linearized approximation of the same discrepancy. Once, the sample point is selected, the weights themselves can be optimized. We name this algorithm (solving linearized discrepancy + optimizing weights) as WKH. For the case when the weights are constrained to sum up to $1$,~\cite{Bach2012Herding} noted that WKH is equivalent to the classic Frank-Wolfe~\cite{Frank1956bt} algorithm on the marginal polytope. 
Exploiting this connection, they were able to use convergence results from Frank-Wolfe analysis to analyze constrained WKH. Specifically, if the optimum lies in the relative interior of the marginal polytope, so that it is distance $b$ away from the boundary, the convergence rate is $O(\exp(-b T))$. 
For finite dimensional kernels, they show $\exists b>0$; while for infinite dimensional kernels, $b=0$. 
Even for finite dimensions, $b$ can be arbitrarily close to $0$, which renders the exponential convergence meaningless.
It was also pointed out by \cite{Bach2012Herding} that the existing theory does not fully justify the much better empirical performance of WKH. To the best of our knowledge, this question has remain unresolved before our present~work.

In our present work, we provide an analysis for exponential convergence of unconstrained WKH. As noted by~\cite{Huszar2012OptimallyWeightedHI}, the weights in WKH do not need to sum to $1$ in many applications, and so the correspondence to Frank-Wolfe and its limitations do not hold for us. Furthermore, our analysis also extends to infinite dimensional kernels, provided a simplifying structural assumption is satisfied. 

Central to our analysis is a novel proof technique that proves linear convergence under a \emph{realizability} assumption. By this, we assume that the mean embedding in the kernel space can be exactly reproduced by a linear combination of $r$ samples $\bx_i, i \in [r]$, from the domain. We discuss the assumption and its impact in Section~\ref{sec:theory}, and we emphasize that it is not restrictive. In fact, for many \emph{nice cases}, $r=1$ or $2$, but more generally, realizability guarantees $O(\exp(-r T))$ convergence. Specifically, it also holds for Stein Kernels~\cite{Gorham2017Stein} which have gained a lot of interest recently because they obviate the need for calculating the target expectation which is often intractable. The comparative view of the algorithms and their respective rates is presented in Table~\ref{tab:Algorithms}.

%A side effect of our analysis is that we are able to scale up the herding algorithm to multiple machines, cutting down on run time and memory requirements. As noted by~\cite{Huszar2012OptimallyWeightedHI}, the $(k+1)^{\text{th}}$ iteration of KH and WKH require an $O(k^2)$ search over the domain to sample the next point, while SBQ requires $O(k^3)$. Thus, for large $k$, these algorithms can get slower. Furthermore, they can be memory intensive. Our proposed solution is to split the domain and hence the search to multiple machines, and to run a \emph{local} WKH/SBQ, thus speeding up the search for the next sample point. The local solutions are then collated to output the final set of samples. Interestingly, we show that this distributed algorithm also exhibits linear convergence under slightly stricter assumptions.
  
%Bach/Lacoste say Herding with uniform weights is bad "converges to max entropy", also noted by Chen/Smola that call the algorithm "chaotic".  

%summary of theretical contributions. 
\begin{table*}[h]
	\centering
	
	\begin{tabular}{|c|c|c|c|}\hline
		Algorithm & Convergence Rate & Setup & Ref. \\\hline 
		MC Integration & $O(1/T)$ & General & - \\
		Kernel Herding & $O(1/T)$ & General & \cite{Chen2010SuperSamples}\\
		Frank-Wolfe & $O(1/T)$ & General & \cite{Bach2012Herding}\\
		Kernel Herding & $O(1/T^2)$ & Finite dimensional kernel & \cite{Chen2010SuperSamples}\\
		Frank-Wolfe & $O(\exp(-T))$ & Finite dim./opt. in rel. interior & \cite{Bach2012Herding}\\
		WKH & $O(\exp(-T))$ & Realizability & (This work)\\
		SBQ & $O(\exp(-T))$ & Realizability & (This work)\\
		Distributed WKH/SBQ &  $O(\exp(-T))$ & Realizability & (This work)\\
		\hline
	\end{tabular}
\caption{Comparative view of the convergence rates of algorithms we consider for the cost $\text{MMD}^2$ (defined in~\eqref{eq:MMDcostfunction}), and related prior work.}
\label{tab:Algorithms}
\end{table*}


%explanation for discrete case, explanation for fast convergence beyond relative interior condition and infinite dimension.
Our contributions in this work are: 
(a) Theoretical---providing the fastest known convergence rates for two popular sampling algorithms; 
(b) Algorithmic---providing a new distributed herding algorithm that we also show converges linearly; and
(c) Empirical---since there is ample empirical evidence supporting the good performance of the KH/SBQ algorithms in earlier works~\cite{Huszar2012OptimallyWeightedHI,Chen2010SuperSamples,Bach2012Herding}, we focus instead on  demonstrating the empirical performance of the distributed algorithm.
In more detail, our main contributions are:\vspace{-0.2cm}
\begin{itemize}
	\item We take a renewed look at convergence analysis through the lens of approximation error after $i$ iterations that is typical in discrete optimization. This allows us to analyze and prove \emph{linear} convergence of two widely used algorithms for approximating expectations, under standard assumptions for well-known setups. Our analysis also provides theoretical justifications for empirical observations already made in the literature. \vspace{-0.1cm}
	
	\item We propose the novel \emph{niceness} assumption of realizability in the optimization problem we study. The assumption trivially holds for many known cases, but even for several harder cases, it acts as a sufficient condition to guarantee linear convergence.\vspace{-0.1cm}
	
	\item We provide a weaker approximation guarantee for cases that do not follow realizability.\vspace{-0.1cm}

	\item We propose a novel \emph{distributed} algorithm for approximating expectations for large scale computations, and we study its convergence properties. To the best of our knowledge, herding has not been applied to such a scale before.\vspace{-0.1cm}
	
	\item Finally, we present \emph{empirical studies} to validate the newly proposed distributed algorithm.\vspace{-0.1cm}
\end{itemize}


%\paragraph{Outline.}
%The rest of the paper is as follows. 
%We present relevant background on the algorithms in Section~\ref{sec:background}. 
%The main theoretical results are presented in Section~\ref{sec:theory}, albeit most of the proofs are relegated to the appendix; and the algorithm for distributed kernel herding is presented in Section~\ref{sec:Distributed}. 
%Finally, we provide empirical results in Section~\ref{sec:Experiments}; and we provide a brief conclusion in Section~\ref{sec:Conclusion}.

==> Theory.tex <==
\section{Convergence Results} \label{sec:theory}

In this section, we establish linear convergence of WKH. The starting point of our analysis is the following re-interpretation of the posterior variance minimization~\eqref{eq:sbq_costfunction} as a variational optimization of Mean Maximum Discrepancy (MMD)~\cite{Huszar2012OptimallyWeightedHI}. We can re-write~\eqref{eq:sbq_costfunction} as a function of a set of chosen sample indices $\sfS$ and weights $\bw$ as: 
\vspace{-2mm}
\begin{eqnarray}\vspace{-4mm}
\label{eq:MMDcostfunction}
g(\sfS, \bw) := \| \mu_p - \sum_{i \in \sfS} w_i \phi(\bx_i) \|_k^2,
\vspace{-2mm}
\end{eqnarray}
where $\phi$ is the respective feature mapping, i.e., $k(\bx,\by) = \langle \phi(\bx), \phi (\by) \rangle$, and where $\mu_p : = \int_{\by \sim p} \phi(\bx) p(\bx)d\bx $ is the mean embedding in the kernel space. We use $\sfS$ to represent the sample indices and samples themselves interchangeably. %In the above discussion, we have implicitly assumed, that the function lies within the chosen RKHS. If that is not the case, $g(\cdot)$ will be the discrepancy 

Before presenting our result, we delineate the assumptions we make on the cost function~\eqref{eq:MMDcostfunction}. There is an implicit assumption that the function under consideration $f(\cdot)$ lies within the chosen RKHS, otherwise there is no guarantee that any algorithm can approximate $f(\cdot)$ within $\epsilon$ error, and the discussion of convergence rates is meaningless. Other assumptions follow.

\paragraph{Assumption 1 (Realizability):} We assume $\exists$ a set $\sfS^\star_r$ of $r$ atoms such that  $\min_\bw g(\sfS^\star_r, \bw) = 0$. 

\emph{Discussion:} Assumption 1 posits there exists a set of samples in the mapped domain $\phi(\cX)$ whose weighted average exactly evaluates to the expectation $\mu_p$ so that the discrepancy $g(\cdot)$ is $0$. 
We emphasize that this assumption is not restrictive. For example, for $d$-dimensional kernels, $r \leq d$, simply because the weights allow linear combination. For Stein Kernels~\cite{Stein1986,barbour_1988,Liu2016KSD,Liu2017Blackbox,Gorham2017Stein}, $\mu_p=0$, and so the assumption trivially holds with $r=1$. However, it turns out we can do a lot better. %Note that the fact that the weights $w_i$ are a linear combination, as opposed to a convex one, is crucial for this trivial result. 

\begin{proposition}\label{prop:realizability}
	Say the domain $\cX$ is compact and continuous, and the mapping $\phi(\cdot)$ is continuous. Further, if the mapped support $\phi(\cX)$ of $p$ is \vspace{-0.2cm}
	\begin{enumerate}
		\item[(a)] convex, then  Assumption 1 holds with $r=1$.
		\item[(b)] non-convex, then Assumption 1 holds with $r=2$.
	\end{enumerate}
\end{proposition}

The proof of Prop~\ref{prop:realizability} relies on the fact that the expectation over a distribution supported on a set would lie within the convex hull of the set. For ease of exposition, the proof is relegated to the Section~\ref{sec:proofPropRealizability}. 

%Consider the simple case for finite dimensional kernels and convex support $\phi(\cX)$. Then, the expectation will lie within $\cX$. Hence, just from continuity properties, the average~\eqref{eq:approxexpectation} must be obtained somewhere on the domain for some $\bx \in \cX$, and so $r=1$. For non-convex $f(\cdot)$, the expectation might lie outside $\cX$, but a linear combination of small $r$ number of points in $\cX$ may still reproduce this value. 
For the cases not covered by the assumptions made in Prop~\ref{prop:realizability} e.g.. discrete $p$, and/or for infinite dimensional $\phi$ with non-compact $\cX$, as long as Assumption 1 is satisfied and can be proved to be so through other means, our work shows that it is sufficient to prove linear convergence. To the best of our knowledge, such a sufficient condition for these harder cases has not been established before, and this is one of our contributions of this work. 

%We conjecture that a similar convergence result could possibly be derived for Frank-Wolfe type algorithms with as assumption similar to Assumption 1, since linear convergence of forward only (i.e. without Away steps) Frank-Wolfe is still an open problem to the best of our knowledge. 

We assume that the loss function $g(\cdot)$ is $m_\omega$-restricted strongly convex and $M_\Omega$-smooth over $\sfS^\star_\perp \cup \sfS_n$, with $m_\omega > 0$ and $M_\Omega < \infty$. In other words, for $\sfS_1, \sfS_2 \subset \sfS_r^\star \cup \sfS_n$, with $Z(\sfS_j) = \sum_j w_j \phi(\bx_j)$, $Z_{12} = Z(\sfS_1) - Z(\sfS_2)$, and $D(\sfS_1, \sfS_2) =g(\sfS_1) - g(\sfS_2)- \langle \nabla g(\sfS_2), Z(\sfS_1) - Z(\sfS_2) \rangle_k $,

\begin{eqnarray*}
     \frac{m_\omega}{2} \| Z_{12}\|_k^2 \leq  D(\sfS_1, \sfS_2)   \leq   \frac{M_\Omega}{2} \| Z_{12} \|_k^2 .
\end{eqnarray*}

% In other words, for $\sfS_1, \sfS_2 \subset \sfS_r^\star \cup \sfS_n$, with $Z(\sfS_j) = \sum_j w_j \phi(\bx_j)$ and $D(\sfS_1, \sfS_2) =g(\sfS_1) - g(\sfS_2)- \langle \nabla g(\sfS_2), Z(\sfS_1) - Z(\sfS_2) \rangle_k $,
%
%\begin{eqnarray*}
%	 \frac{m_\omega}{2} \| Z(\sfS_1) - Z(\sfS_2) \|_k^2 &\leq&  D(\sfS_1, \sfS_2) \\&  \leq & \frac{M_\Omega}{2} \| Z(\sfS_1) - Z(\sfS_2) \|_k^2 .
%\end{eqnarray*}

% eigenvalues of the kernel matrix formed by applying the kernel function on  are lower bounded by $m_\omega>0$ and upped bounded by $M_\Omega < \inf$.


Assumption 2 is standard when it comes to characterizing geometric rates in optimization e.g. see~\citep{wainwright2019high} (Section 9.3.1), and is often implicitly assumed e.g. by~\cite{Bach2012Herding}. This assumption or a slight variation of it, is only sufficient but also necessary to bound geometric convergence rates. For our case, one can equivalently view the assumption as stating that the kernel matrix of the atoms $\sfS^\star_\perp \cup \sfS_n$ has lower eigenvalue bounded away from $0$ for any fixed $n$, since we are interested in non-assymptotic convergence rates.  Note that as $n \rightarrow \infty$, it may seem like characterizing the lower bound of $m_\omega$ requires taking a uniform bound over the entire support of $p$, as is typically done in classical optimization. However, by virtue of the algorithm's design, more specifically because of the weights $w_i$ being allowed to be linear combination of the selected atoms, any new atom being added would not lie within the span of already selected atoms. As such, the kernel matrix of the chosen atoms would always have its lower eigenvalue bounded away from $0$, which implies that $m_\omega$ stays greater than $0$ as $n$ grows unless no more atoms can be added.


% function~\eqref{eq:MMDcostfunction}.  %One can take a uniform bound to make a simpler (albeit a lot stricter) assumption of strong convexity and smoothness to hold over the entire domain. 

\paragraph{Assumption 3 (Standardization):} We assume that the feature mapping is standardized, i.e., $k(\bx,\bx) = 1 \, \forall \bx \in \cX$, as assumed in previous works~\cite{Huszar2012OptimallyWeightedHI}, for ease of exposition. 

Assumption 3 is not restrictive. It is only presented in order to avoid unnecessary complications that distract from our main message. It is well-known that any kernel can be normalized. e.g. normalized linear kernel is the cosine kernel. While it may look like that normalization is changing the kernel, it is merely zeroing out effect of individual norms of atoms so that the atoms with larger norms do not dominate the selection process, and allowing the selection based on relationships amongst atoms which is what herding/quadrature algorithms care about. 

Assumptions 1 through 3 are satisfied by many commonly used kernels. From Proposition~\ref{prop:realizability}, any finite dimensional normalized kernel (e.g. cosine kernel, polynomial kernels etc.) or general normalized kernels on compact supports and continuous $p$ (e.g. stein kernels, RBFs, Matern kernels) satisfy them. For discrete $p$, as the number of candidate atoms $N \rightarrow \infty$, the assumptions are satisfied with probability 1.  We are now ready to present our main result regarding the linear convergence of the discrepancy metric $g(\cdot)$.
\begin{theorem}
	\label{thm:WKHLinear} Under Assumptions 1 through 3, if $\sfS_i$ is the sequence of iterates produced by Algorithm~\ref{algo:wkh}, the function $g(\cdot)$ converges as $\min_w g(\sfS_i, \bw) \leq \exp(- \frac{i m_\omega}{r M_\Omega}) g(\emptyset, 0)$.
\end{theorem} 

\noindent
%\emph{Proof Outline.} The central idea of the proof is to track and bound the selection of a sample at each iteration, compared to the ideal selection $\sfS^\star_r$ that could have provided the optimum solution. For this purpose, the properties of the selection subproblem~\eqref{eq:LMO} and the assumptions are  used. The detailed proof is presented in the appendix.

\emph{Discussion:} Theorem~\ref{thm:WKHLinear} provides a linear convergence rate for \wkh~ under the sufficient conditions specified in Assumptions 1 through 3.~\cite{Bach2012Herding} also provided a linear rate for finite dimensional kernels by drawing on the equivalence of the herding algorithm to the Frank-Wolfe algorithm. Their rate is $O(\exp{(-b^2T/R^2)})$, where $b$ is the distance of the optimum from the boundary of the marginal polytope and $R$ is the width of the marginal polytope. Our result is independent of these constants; and by Proposition~\ref{prop:realizability}, is better than their rates, as long as $\frac{R}{b} > \sqrt{2}$ for finite dimensional kernels. Since $b$ can be arbitrarily close to $0$, our results are much stronger and more general in the sense that they are independent of where the optimum lies. Furthermore, our results will hold for infinite dimensional kernels, as long as the above mentioned sufficient conditions are satisfied. 

\paragraph{Relationship with SBQ}
%The SBQ Algorithm~\cite{Ghahramani2002BayesianMC,Huszar2012OptimallyWeightedHI} is similar to the WKH algorithm, except that it solves a slightly more involved optimization subproblem to select the next sample point. 
The SBQ pseudocode is exactly the one presented in Algorithm~\ref{algo:wkh}, with step 4 replaced with~\eqref{eq:LMO_SBQ} instead of~\eqref{eq:LMO}. 
Thus, WKH solves a linear program every iteration, while SBQ solves a kernel $\ell_2$ minimization problem. 
%In this and other theoretical work, it is assumed that the oracle that solves the optimization subproblem is given and the convergence rates generally consider the number of calls made to this oracle for desired accuracy of the overall solution. 
%In applications, however, the subproblems can be vastly impactful on convergence, run times, and memory management. 
%It has been observed that SBQ converges faster in practice, which is intuitive since it performs more work \emph{per iteration}. 
%Furthermore, for distributed algorithm variants like the one presented in Section~\ref{sec:Distributed}, the cost per iteration may not be a bottleneck due to availability of multiple machines. 
%On the other hand, in addition to higher cost per iteration, the application of SBQ might not be always feasible. 
%We present one such example in Section~\ref{sec:Experiments}, where SBQ requires memorization of the kernel matrix for a reasonable run time. 
The decrease in the cost function~\eqref{eq:MMDcostfunction} per iteration of SBQ is more than its decrease per iteration of WKH. This relationship, combined with Theorem~\ref{thm:WKHLinear} establishes geometric convergence of SBQ, which to the best of our knowledge, was still an open question (see Table 1 in~\cite{Huszar2012OptimallyWeightedHI} which lists the convergence rate of SBQ as \emph{unknown}).

\begin{corollary}
	\label{cor:convergenceSBQ} Under Assumptions 1 through 3, if $\sfS_i$ is the sequence of iterates produced by SBQ, the function $g(\cdot)$ converges as $\min_\bw g(\sfS_i, \bw) \leq \exp(- \frac{i m_\omega}{r M_\Omega}) g(\emptyset, 0)$.
\end{corollary}

\subsection{Breaking realizability}
\label{sec:breaking_realizability}

 While realizability holds with $r\leq 2$ for many \emph{nice cases}, it is important to discuss cases when realizability breaks. Consider the case of discrete $p$. Say  $n$ is the size of the support of discrete $p$, and $d$ is the dimensionality of the kernel space. If $n \gg d$, from the fact that each iteration only adds an atom that is in the orthogonal complement of previously added samples, $r \leq d$.
In this case, the same rate will still hold. 
On the other hand, it is possible that the mean $\bbE_p(f)$ is realizable for no less than $r = O(n)$ samples if $d \approx n$. 
In this case, the linear rate is no longer valid. 
One can call upon the Frank-Wolfe connection~\cite{Bach2012Herding}, since as long as $d < \infty$, we know that the a linear rate holds (because the optimum lies in the relative interior away from the boundary, since the effective rate is minimum of the two). 
However, as discussed before, the optimum may lie arbitrarily close to the boundary. In such cases, the following statement still holds nonetheless.

\begin{theorem}\label{thm:approx} (Approximation guarantee) Say Assumptions 2 and 3 are satisfied. Let $\sfT_r := \argmin_{|\sfS| \leq r} \min_\bw g(\sfS,\bw)$. Say $k=(r \frac{M_\Omega}{m_\omega}\log \frac{1}{\epsilon})$ iterations of Algorithms~\ref{algo:wkh} (WKH or SBQ) select the set $\sfS_k$. Then, $ \min_\bw g(\sfS_k, \bw) ) \leq (1- \epsilon) [ \min_\bw g(\sfT_r, \bw)] + \epsilon \| \mu_p\|_k^2 $. 
\end{theorem}
	
The proof is presented in Section~\ref{sec:appendixApproxGuaranteeProof}.  Theorem~\ref{thm:approx} is weaker than a convergence result but it also makes weaker assumptions since it does not need Assumption 1.  Instead of providing a rate on how close we are to the optimum after $k$ iterations, it provides a contraction factor on how close the algorithm gets to the best possible $r$ steps that \emph{any} algorithm could have taken. This recovers the special case of SBQ for discrete densities studied by~\cite{Khanna2019} by exploiting connections to weak submodularity. Their result is also an approximation guarantee (not global convergence guarantee), and only applies for SBQ. Our result is also valid for WKH and provides an alternative proof for SBQ without exploiting weak submodularity. Also note that we also recover the geometric contraction for Stein Kernels which have $\mu_p =0$ from Theorem~\ref{thm:approx}.
%
%Theorem~\ref{thm:approx} is valid for infinite dimensional kernel spaces as well. It is possible that in infinite dimensions,  $\bbE_P(f)$ is not realizable for any $r < \infty$. We characterize this as a \emph{pathological case}, since it implies that $\bbE_P(f)$ is not in the span of any finite number of atoms $\bx_i$. One can, however, provide the following weaker guarantee. For any projection of $\bbE_P(f)$ onto a finite number of atoms $r$, we need to run atmost $O(r \log \frac{1}{\epsilon})$ iterations of Algorithms~\ref{algo:wkh} (WKH or SBQ), in order to get $\epsilon$ close to the objective value of the best such  $r$-sized projection.  

%Another implicit assumption made by the sampling algorithms we consider is that the function $f(\cdot)$ lies within the chosen RKHS, which may not always be the case. However, if that is the case, the cost function~\ref{eq:MMDcostfunction} can be considered as minimizing the projection

